Fast Underwater Image Enhancement for Improved Visual Perception

In this paper, we present a conditional generative adversarial network-based model for real-time underwater image enhancement. To supervise the adversarial training, we formulate an objective function that evaluates the perceptual image quality based on its global content, color, local texture, and style information. We also present EUVP, a large-scale dataset of a paired and unpaired collection of underwater images (of `poor' and `good' quality) that are captured using seven different cameras over various visibility conditions during oceanic explorations and human-robot collaborative experiments. In addition, we perform several qualitative and quantitative evaluations which suggest that the proposed model can learn to enhance underwater image quality from both paired and unpaired training. More importantly, the enhanced images provide improved performances of standard models for underwater object detection, human pose estimation, and saliency prediction. These results validate that it is suitable for real-time preprocessing in the autonomy pipeline by visually-guided underwater robots. The model and associated training pipelines are available at https://github.com/xahidbuffon/funie-gan.

==> src/head.tex <==
\usepackage{graphicx} % for pdf, bitmapped graphics files
\usepackage{subcaption}
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed https://preview.overleaf.com/public/rsfmwkfvqdyp/images/8e680429ab22701a0e03ee380cd8785b240c35ed.jpeg
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
%\usepackage{svg}
%\usepackage{dsfont}
%\usepackage{hyperref}
\usepackage{csquotes}
\def\UrlBreaks{\do\/\do-}

\usepackage{array}
\usepackage{url} 
\usepackage{enumerate}
%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{multirow} % tables
%\usepackage{rotating} % for rotating texts
%\usepackage{subfigure}
\usepackage{float}
\usepackage{paralist}
\usepackage{amsfonts}
%\pagestyle{empty} % hiding page numbering
\sloppy % for tricky allignments
%\usepackage[justification=centering]{caption}
\usepackage{longtable}

%\usepackage{algorithmic}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Junaed's definition of a sidenote to look into
\newcommand{\marginlabel}[1]{\mbox{}\marginpar[\raggedleft\hspace{0pt}{#1}]{
		\raggedright\hspace{0pt}{#1}}}
\graphicspath{ {images/} }
\newcommand{\starnote}[1]{\marginlabel{$\bigstar$}\textbf{[#1]}}
% comment the previous line and uncomment the one below to remove all such notes in the output PDF
\newcommand{\nostarnote}[1]{}
\newcommand{\baad}[1]{} 
\usepackage[size=small]{caption}
%\usepackage{enumitem}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\etal}{\textit{et al.}} 
